DeepCache: Principled Cache for Mobile Deep Vision

We present DeepCache, a principled cache design for deep learning inference in continuous mobile vision. DeepCache benefits model execution efficiency by exploiting temporal locality in input video streams. It addresses a key challenge raised by mobile vision: the cache must operate under video scene variation, while trading off among cacheability, overhead, and loss in model accuracy. At the input of a model, DeepCache discovers video temporal locality by exploiting the video's internal structure, for which it borrows proven heuristics from video compression; into the model, DeepCache propagates regions of reusable results by exploiting the model's internal structure. Notably, DeepCache eschews applying video heuristics to model internals which are not pixels but high-dimensional, difficult-to-interpret data. Our implementation of DeepCache works with unmodified deep learning models, requires zero developer's manual effort, and is therefore immediately deployable on off-the-shelf mobile devices. Our experiments show that DeepCache saves inference execution time by 18% on average and up to 47%. DeepCache reduces system energy consumption by 20% on average.

==> secs/lst-api.tex <==
\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}
\lstset{frame=tb,
  language=Java,
  aboveskip=3mm,
  belowskip=3mm,
  showstringspaces=false,
  columns=flexible,
  basicstyle={\small\ttfamily},
  numbers=left,
  numberstyle=\tiny\color{gray},
  keywordstyle=\color{blue},
  commentstyle=\color{dkgreen},
  stringstyle=\color{mauve},
  breaklines=true,
  breakatwhitespace=true,
  tabsize=3,
  xleftmargin=0.5cm
}
\begin{lstlisting}[caption={APIs of using \framework}, label={list:javaSample}]
COMO infer = new COMO("/path/to/model"); // Initialize a runtime from pre-trained model
infer.enable_cache(true); // (Optional) default true
infer.set_psnr_threshold(25); // (Optional) Set the threshold for image matching, default 20
infer.set_block_size(15); // (Optional) default 10
infer.set_expire(10); // (Optional) default 10
infer.run(input_name, input_data);
float[] result = infer.fetch(output_name);
\end{lstlisting}

==> secs/tab-loc.tex <==
\begin{table}
\normalsize
\centering
\begin{tabular}{llr} \hline
	\textbf{Module} & \textbf{Language} & \textbf{LoC}\\ \hline
	Caching inside \emph{ncnn} & C/C++ & 3,620\\
	Image matching & Java, rs & 410\\
	\textit{Total} & & \textit{4,030}\\ \hline
\end{tabular}
\caption{LoC (Lines of Code) of \framework.}
\label{tab:LoC}
\end{table}
